Combining Gesture and Voice Control for Mid-Air Manipulation of CAD Models in VR Environments

Modeling 3D objects in domains like Computer Aided Design (CAD) is time-consuming and comes with a steep learning curve needed to master the design process as well as tool complexities. In order to simplify the modeling process, we designed and implemented a prototypical system that leverages the strengths of Virtual Reality (VR) hand gesture recognition in combination with the expressiveness of a voice-based interface for the task of 3D modeling. Furthermore, we use the Constructive Solid Geometry (CSG) tree representation for 3D models within the VR environment to let the user manipulate objects from the ground up, giving an intuitive understanding of how the underlying basic shapes connect. The system uses standard mid-air 3D object manipulation techniques and adds a set of voice commands to help mitigate the deficiencies of current hand gesture recognition techniques. A user study was conducted to evaluate the proposed prototype. The combination of our hybrid input paradigm shows to be a promising step towards easier to use CAD modeling.

==> sections/conclusion.tex <==
\section{\uppercase{Conclusion}}
\label{sec:concept}

In this work, a novel mid-air manipulation technique, based on CSG structures of objects, was presented. 
To make the interaction as simple and intuitive as possible to the user, the developed application is based on three control elements: Unimanual gesture controls via the demonstrated virtual handle, voice control, and a virtual widget we named the tree tool. 
We conducted a qualitative user study, which showed that users learn and understand our manipulation method very quickly.

Manipulations based on the CSG structure seem to be a reasonable option. 
All participants were able to quickly recognize the structure of small objects.
The more complex an object became, and the smaller its primitives were, the more difficult this process got. 
This means our technique is particularly applicable to the manipulation of simple rather coarse objects.

Furthermore, we want to state out that the tree tool is an intuitive tool that helps users to easily identify the structure of an object. 

Also, DOF separation and the possibility to interact with the voice control seem to be a promising combination. 
It turned out to be beneficial that the users did not have to move their hands to change transformation. 
However, voice control must work very well to avoid user frustration. Unfortunately, this was not always the case in our conducted user studies.

Moreover, our study shows that the virtual handle is also very well suited for virtual reality. 
The users are able to gain a full understanding of the functionality without further explanation and indicate that they find both translating and scaling easy and intuitive. 
